Aerodynamic Control of Laminar Separation on a Wall-Bounded Airfoil at Transitional Reynolds Numbers

Experiments were conducted in a low-turbulence wind tunnel to investigate the efficacy of localised acoustic forcing upon the dynamics and stability of the flow on a cambered, wall-bounded airfoil over a range of Reynolds numbers (Re) where the flow state can switch between two limits -- a low-lift state (SI) where separation continues beyond the trailing edge and a high-lift state (SII) where the separated flow is closed off to form a laminar separation bubble. The switching between SI and SII can occur close to a critical angle of attack ($\alpha_{\textrm{crit}}$) which varies with $\textrm{Re}$. The most effective forcing frequencies are found at a constant value of a rescaled Strouhal number, $\textrm{St}^* = \textrm{St}/\textrm{Re}^{1/2}= 0.027$, which indicates that though the primary unstable modes of the separated shear layer are of the inviscid, Kelvin-Helmholtz type, these modes are seeded by length scales that originate in the laminar (viscous) boundary layer. The most effective chordwise forcing location varies with $\textrm{St}/\textrm{Re}^{1/2}$ and incidence angle, $\alpha$, and is always upstream of the separation point. Although the boundary layer flows are far from two-dimensional, forcing at a fixed chord location across all spanwise locations is effective in controlling the SI -- SII transition. Strategies for active and passive feedback control are suggested.

==> sections/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Wind tunnel experiments on a wall-bounded NACA 65(1)412 airfoil with spanwise distributed speakers embedded inside its suction surface, at a given chordwise location, demonstrated improvements of $L/D$ greater than $90\%$. Coherent trends in forcing frequency and chordwise forcing location were observed. Optimal frequencies and locations were identified and related to flow phenomena from baseline flow field measurements for each Re. Force measurements and separation location estimates were compared with previous experiments and DNS. Reasonable agreement was found between the datasets with the largest discrepancies occurring due to differences in critical angle of attack ($\alpha_\text{crit}$). Further study of the effects of Re and $\alpha$ on the onset and growth rate of the laminar boundary instability are warranted to fully understand the physics behind optimal forcing location, yet the results here show effective control strategies for material improvement in airfoil performance at transitional Re.
